Unsupervised Doppler Radar-Based Activity Recognition for e-Healthcare

Passive radio frequency (RF) sensing and monitoring of human daily activities in elderly care homes is an emerging topic. Micro-Doppler radars are an appealing solution considering their non-intrusiveness, deep penetration, and high-distance range. Unsupervised activity recognition using Doppler radar data has not received attention, in spite of its importance in case of unlabelled or poorly labelled activities in real scenarios. This study proposes two unsupervised feature extraction methods for the purpose of human activity monitoring using Doppler-streams. These include a local Discrete Cosine Transform (DCT)-based feature extraction method and a local entropy-based feature extraction method. In addition, a novel application of Convolutional Variational Autoencoder (CVAE) feature extraction is employed for the first time for Doppler radar data. The three feature extraction architectures are compared with the previously used Convolutional Autoencoder (CAE) and linear feature extraction based on Principal Component Analysis (PCA) and 2DPCA. Unsupervised clustering is performed using K-Means and K-Medoids. The results show the superiority of DCT-based method, entropy-based method, and CVAE features compared to CAE, PCA, and 2DPCA, with more than 5\%-20\% average accuracy. In regards to computation time, the two proposed methods are noticeably much faster than the existing CVAE. Furthermore, for high-dimensional data visualisation, three manifold learning techniques are considered. The methods are compared for the projection of raw data as well as the encoded CVAE features. All three methods show an improved visualisation ability when applied to the encoded CVAE features.

==> 4_Discussion.tex <==
\section{Discussion}
The confusion matrices for the CVAE-based architecture in Figure \ref{fig:cm} reveal that the activities Walking (1) and Jumping (3) are problematic as they are frequently confused. Similarly, the architecture GLCM+K-Means and GLCM+K-Medoids in Figure \ref{fig:cm_glcm} also show confusion between Walking (1) and Jumping (3). In addition to this, the Standing (5) activity is recognised as Running (2) in all cases as the second architecture suffers from poorer average testing accuracies.

Considering the two proposed architectures, it can be concluded that CVAE+K-Means and CVAE-K-Medoids is superior in comparison with GLCM+K-Means and GLCM-K-Medoids for feature extraction. On the other hand, the GLCM-based model is less complex and it is more easily implemented. As a whole, the recognition performance for both architectures is reasonable, which can be applied to other unsupervised project scenarios.

The three manifold learning methods considered in this study can be extremely useful in data visualisation problems.
